An Analysis of $D^\alpha$ seeding for $k$-means

One of the most popular clustering algorithms is the celebrated $D^\alpha$ seeding algorithm (also know as $k$-means++ when $\alpha=2$) by Arthur and Vassilvitskii (2007), who showed that it guarantees in expectation an $O(2^{2\alpha}\cdot \log k)$-approximate solution to the ($k$,$\alpha$)-means cost (where euclidean distances are raised to the power $\alpha$) for any $\alpha\ge 1$. More recently, Balcan, Dick, and White (2018) observed experimentally that using $D^\alpha$ seeding with $\alpha>2$ can lead to a better solution with respect to the standard $k$-means objective (i.e. the $(k,2)$-means cost). In this paper, we provide a rigorous understanding of this phenomenon. For any $\alpha>2$, we show that $D^\alpha$ seeding guarantees in expectation an approximation factor of $$ O_\alpha \left((g_\alpha)^{2/\alpha}\cdot \left(\frac{\sigma_{\mathrm{max}}}{\sigma_{\mathrm{min}}}\right)^{2-4/\alpha}\cdot (\min\{\ell,\log k\})^{2/\alpha}\right)$$ with respect to the standard $k$-means cost of any underlying clustering; where $g_\alpha$ is a parameter capturing the concentration of the points in each cluster, $\sigma_{\mathrm{max}}$ and $\sigma_{\mathrm{min}}$ are the maximum and minimum standard deviation of the clusters around their means, and $\ell$ is the number of distinct mixing weights in the underlying clustering (after rounding them to the nearest power of $2$). We complement these results by some lower bounds showing that the dependency on $g_\alpha$ and $\sigma_{\mathrm{max}}/\sigma_{\mathrm{min}}$ is tight. Finally, we provide an experimental confirmation of the effects of the aforementioned parameters when using $D^\alpha$ seeding. Further, we corroborate the observation that $\alpha>2$ can indeed improve the $k$-means cost compared to $D^2$ seeding, and that this advantage remains even if we run Lloyd's algorithm after the seeding.

==> ImprovedUpperBound.tex <==
We assume all the clusters satisfy the following concentration condition:

We also denote by $\smax$ and $\smin$ the maximum and minimum variance of any cluster $C$ around its mean $\mu_C$. We also do geometric grouping of the mass classes. The set $\mathcal M_i$ is defined to contain all the clusters of mass in the interval $[2^i,2^{i+1})$ (for any $i\ge 0$). We denote by $k_i$ the number of clusters in $\mathcal M_i$. We also define $k_i$ to be the number of clusters in $\mathcal M_i$. The set of indices $i\ge 0$ such that $k_i>0$ is denoted by $\mathcal L$, with $\ell:=|\mathcal L|$.

The goal of this section is to prove the following theorem.





We define the integer $t\ge 0$ as the current time (i.e. the number of centers we selected so far). For each $i\ge 0, t\ge 0$, we also define a integer $\tau_i(t)\ge 0$ which will be a local timer, relevant only for the clusters in $\mathcal M_i$ at time $t$. 


At time $t$, we define $Z_t$ to be the set of selected centers so far, $z_t$ the center selected at timestep $t$, $H_t$ set of hit clusters, and $U_t^{(i)}$ the set of undiscovered clusters in class $\mathcal M_i$. For each $i\ge 0$ and time $t$, we will define an integer $w_i(t)\ge 0$ corresponding to the number of iterations that are considered wasted by the class $\mathcal M_i$ at time $t$.

We initialize $t=0$, $w_i(0)=0$ for all $i$, and $\tau_i(0)=0$ for all $i$.

Then, we maintain these quantities as follows. At time $t\ge 0$, let $C$ be the cluster the next center $z_t$ is chosen from. Let $i\ge 0$ be the integer such that $C\in \mathcal M_i$. Then, there are three cases. 

If $C\in U_t^{(i)}$, then we set

\begin{equation*}
    \tau_j(t+1)=
    \begin{cases}
        \tau_j(t)+1 \mbox{ if $j=i$ and $\tau_j(t)<k_i$}\\
        \tau_j(t) \mbox{ if $j=i$ and $\tau_j(t)\ge k_i$}\\
        \tau_j(t) \mbox{ if $j\neq i$,}
    \end{cases}
\end{equation*}
and $w_j(t+1)=w_j(t) $ for all $j\ge 0$. Otherwise if $C\in H_t$, then we set 
\begin{equation*}
    \tau_j(t+1)=
    \begin{cases}
        \tau_j(t)+1 \mbox{ if $\tau_j(t)<k_i$}\\
        \tau_j(t) \mbox{ if $\tau_j(t)\ge k_i$,}\\
    \end{cases}
\end{equation*}
and 
\begin{equation*}
    w_j(t+1)=
    \begin{cases}
        w_j(t)+1 \mbox{ if $w_j(t)<k_i$}\\
        w_j(t) \mbox{ if $w_j(t)\ge k_i$.}\\
    \end{cases}
\end{equation*}

Based on these quantities, we define the potential function as follows. First, we define
\begin{equation*}
    \phi_i(t) := \frac{w_i(t)}{|U_t^{(i)}|} \cdot (2^i)^{1-2/\alpha} \cdot \sum_{C\in U_t^{(i)}} (\costa (C,Z_t))^{2/\alpha}\ .
\end{equation*}
The final potential function can now be defined as 
\begin{equation*}
    \phi(t) = \sum_{i\ge 0} \phi_i(t)\ .
\end{equation*}

To analyze the sampling algorithm, we need a few crucial lemmas.
\begin{lemma}
%\label{lem:number_of_tries}
    For all $i\ge 0$, we have that $w_i(k)\ge|U_k^{(i)}|$.
\end{lemma}
\begin{proof}
    Consider the quantity $\delta_i(t):=|U_t^{(i)}|-w_i(t)$. Clearly, we have that $\delta_i(0)=k_i$. Next, notice that for every time-step $t<k$ such that $\tau_i(t+1)=\tau_i(t)$, the quantity $\delta_i(t)$ decreases by $1$. Indeed, either the algorithm discovers a new cluster in $|U_t^{(i)}|$ (in which case $|U_{t+1}^{(i)}|=|U_t^{(i)}|-1$), or the algorithms wastes an iteration in some cluster, in which case $w_i(t+1)=w_i(t)+1$. 
    
    Finally, we claim that there are at least $k_i$ such iterations. Note that if $\tau_i(t)<k_i$, then the only way we have that $\tau_i$ does not increase is if the algorithm discovers a new cluster in $|U_t^{(j)}|$ for some $j\neq i$. This can happen at most $\sum_{j\neq i} k_j$ times. Hence there must be at least $k-\sum_{j\neq i} k_j=k_i$ iterations where the counter $\tau_i$ increases. If we denote by $t_i$ the first time at which $\tau_i(t_i)=k_i$, this implies $t_i\le k$ and that that $\delta_i(t_i)=0$ hence $w_i(t_i)=U_{t_i}^{(i)}$. Finally, note that for $t>t_i$ $w_i(t)$ does not change anymore, and $|U_t^{(i)}|$ can only decrease; which concludes the proof.
\end{proof}

\begin{lemma}
%\label{lem:potential_upper_bound}
    We have that $\phi_k \ge \sum_{i\ge 0}\cost (U_k^{(i)},Z_k)/2=\cost (U_k,Z_k)/2$.
\end{lemma}
\begin{proof}
    Using Lemma \ref{lem:number_of_tries}, we have that 
    \begin{equation*}
        \phi(k)=\sum_{i\ge 0}\phi_i(k)\ge (1/2)\cdot (2^{i+1})^{1-2/\alpha} \cdot \sum_{C\in U_k^{(i)}} (\costa (C,Z_k))^{2/\alpha}\ .
    \end{equation*}
    Using Jensen's inequality and the fact that $|C|\le 2^{i+1}$ for all $C\in U_k^{(i)}$, we have that $(2^{i+1})^{1-2/\alpha}(\costa (C,Z_k))^{2/\alpha} \ge \cost(C,Z_k)$ for all $C\in U_k^{(i)}$, which concludes the proof.
\end{proof}

\begin{lemma}
\label{lem:potential_hit_new}
Let $A_t^{(i)}$ be the event that the $t$-th center is selected from and undiscovered cluster belonging to mass class $i$. Then, for any $t> 0$, $i,j\ge 0$, any past choice of centers $Z_{t-1}$, we have that 
\begin{equation*}
    \mathbb E\bigg[\phi_j(t)-\phi_j(t-1) \mid \{Z_{t-1}, A_t^{(i)}\}\bigg] \le 0.
\end{equation*}
\end{lemma}
\begin{proof}
    We first note that since $z_t\notin H_t$, it is clear that $\phi_j(t)\le \phi_j(t-1)$ for all $j\neq i$. To bound the change of $\phi_i$ we notice that $w_i(t)=w_i(t-1)$, and that $|U_t^{(i)}|=|U_{t-1}^{(i)}|-1$. Let $C_z$ be the cluster which is selected in $U_{t-1}^{(i)}$. We claim that 
    \begin{equation}
        \mathbb E\bigg[(\costa(C_z,Z_{t-1}))^{2/\alpha} \mid  \{Z_{t-1}, A_t^{(i)}\}\bigg] \ge \frac{1}{|U_{t-1}^{(i)}|}\cdot \sum_{C\in U_{t-1}^{(i)}}(\costa(C,Z_{t-1}))^{2/\alpha}\ .
    \end{equation}
    Indeed, note that 
    \begin{align*}
       \E\left[(\costa(C_z,Z_{t-1}))^{2/\alpha}\mid \{Z_{t-1}, A_t^{(i)}\} \right]&=\sum_{C \in U_{t-1}^{(i)}}\frac{\costa(C,Z_{t-1})}{\sum_{C \in U_{t-1}^{(i)}}\costa(C,Z_{t-1})}\cdot\left(\costa(C,Z_{t-1})\right)^{2/\alpha}\\
       &\hspace{-20mm}=\frac{|U_{t-1}^{(i)}|}{\sum_{C \in U_{t-1}^{(i)}}\costa(C,Z_{t-1})}\cdot \sum_{C \in U_{t-1}^{(i)}}\frac{\costa(C,Z_{t-1})\cdot\left(\costa(C,Z_{t-1})\right)^{2/\alpha}}{|U_{t-1}^{(i)}|}\\
       &\hspace{-20mm}\stackrel{(1)}{\geq} \frac{|U_{t-1}^{(i)}|}{\sum_{C \in U_{t-1}^{(i)}}\costa(C,Z_{t-1})}\cdot \sum_{C \in U_{t-1}^{(i)}}\frac{\costa (C,Z_{t-1})}{|U_{t-1}^{(i)}|}\cdot \sum_{C \in U_{t-1}^{(i)}}\frac{(\costa(C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}\\
       &\hspace{-20mm}=\sum_{C \in U_{t-1}^{(i)}}\frac{(\costa(C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}\ .
   \end{align*}
   The inequality (1) can be obtained Lemma \ref{lem:chebyshevsum} by considering the ordered sequence $\{\costa(C,Z_{t-1})\}_{C\in U_{t-1}^{(i)}}$ and $\{(\costa(C,Z_{t-1}))^{2/\alpha}\}_{C \in U_{t-1}^{(i)}}$. Thus we have:
   \begin{align*}
   &\E\left[\phi_i(t)\mid \{Z_{t-1}, A_{t}^{(i)}\}\right]\\
   &\leq \frac{w_i(t)}{|U_{t-1}^{(i)}|-1} \cdot (2^i)^{1-2/\alpha} \cdot \left( \sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_t))^{2/\alpha} -  \E\left[(\costa_t(C_z,Z_{t-1}))^{2/\alpha}\mid \{Z_{t-1}, A_t^{(i)}\} \right] \right)\\
   &\le \frac{w_i(t)}{|U_{t-1}^{(i)}|-1} \cdot (2^i)^{1-2/\alpha} \cdot \left( \frac{|U_{t-1}^{(i)}|-1}{|U_{t-1}^{(i)}|}\cdot \sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_{t-1}))^{2/\alpha}\right)\\
   &=\phi_i(t-1).
   \end{align*} 
\end{proof}


\begin{lemma}
\label{lem:potential_hit_old}
    Let $B_t$ be the event that the $t$-th center is selected from $H_t$. Then, for any $t> 0$, $i\ge 0$, and any past choice of centers $Z_{t-1}$, we have that 
    \begin{equation*}
    \mathbb E\bigg[\phi_i(t)-\phi_i(t-1) \mid \{Z_{t-1}, B_t\}\bigg] \le (\tau_i(t)-\tau_i(t-1))\cdot \frac{(2^i)^{1-2/\alpha}}{|U_{t-1}^{(i)}|} \cdot \sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_  {t-1}))^{2/\alpha}\ .
\end{equation*}
\end{lemma}
\begin{proof}
    Fix some $i\ge 0$. If $\tau_i(t-1)=\tau_i(t)$, we have by definition $w_i(t)=w_i(t-1)$ and clearly the potential $\phi_i$ cannot increase. Otherwise, we simply note that $w_i(t)=w_i(t-1)+1$, and the result clearly follows.
\end{proof}
\begin{lemma}
    Assume some arbitrary set $T$ of centers have already been selected, and $z\in C$ is added next using $D^\alpha$-sampling. Then,
    \begin{equation*}
        \mathbb  E\left[ \cost(C,T\cup \{z\})\mid z\in C\right]\le (2e+(\alpha+1)^2\cdot (g_\alpha)^{2/\alpha} )\cdot  \cost(C,\mu_C) \ .
    \end{equation*}
\end{lemma}
\begin{proof}
    We can write
    \begin{equation*}
        E\left[ \cost(C,T\cup \{z\})\mid z\in C\right] = \sum_{z\in C} \frac{\costa (z,T)}{\costa (C,T)}\cdot \sum_{x\in C} \min \{\cost (x,T), ||x-z||^2\}\ .
    \end{equation*}
    Let us upperbound the quantity $\costa (z,T)$. For this, let us fix any $x\in C$. Then, if we denote by $t_x$ the point in $T$ which is closest to $x\in C$, we have that 
    \begin{equation*}
        \costa (z,T) \le  ||z-t_x||^\alpha \le (||z-x||+||x-t_x||)^\alpha \le (\alpha+1)^\alpha \cdot ||z-x||^\alpha + (1+1/\alpha)^\alpha\cdot  ||x-t_x||^\alpha\ ,
    \end{equation*}
    using the triangle inequality and a case distinction whether $||z-x||>(1/\alpha) ||x-t_x||$ or not. Averaging this upper bound over all $x\in C$, we obtain that 
    \begin{align*}
        \costa (z,T) &\le \frac{(\alpha+1)^\alpha \cdot \costa(C,z)}{|C|}+\frac{(1+1/\alpha)^\alpha\cdot \costa(C,T)}{|C|}\\
        &\le \frac{(\alpha+1)^\alpha\cdot  \costa(C,z)}{|C|}+\frac{e\cdot \costa(C,T)}{|C|}\ .
    \end{align*}
    Hence we can rewrite 
    \begin{align*}
        \mathbb E&\left[ \cost(C,T\cup \{z\})\mid z\in C\right] \\
        &\le \sum_{z\in C} \frac{\frac{(\alpha+1)^\alpha\cdot  \costa(C,z)}{|C|}+\frac{e\cdot \costa(C,T)}{|C|}}{\costa (C,T)}\cdot \sum_{x\in C} \min \{\cost (x,T), ||x-z||^2\}\\
        &\le \frac{e}{|C|}\sum_{z\in C}  \cost(C,z) + \frac{(\alpha+1)^\alpha}{|C|}\sum_{z\in C} \frac{\costa(C,z)}{\costa (C,T)}\cdot \cost (C,T)\ .
    \end{align*}
    To finish the argument, note that the first term in the last line corresponds to the expected cost of $C$ if we pick once center $z\in C$, uniformly at random. By Lemma \ref{lem:}, this is at most $(2e)\cdot \cost(C,\mu_C)$. For the second term, we use Equation \eqref{eq:concentration_assumption_new} to write 
    \begin{equation*}
        \frac{(\alpha+1)^\alpha}{|C|}\sum_{z\in C} \frac{\costa(C,z)}{\costa (C,T)}\cdot \cost (C,T) \le ((\alpha+1)^\alpha g_\alpha) \cdot  (\cost(C,\mu_C))^{\alpha/2}\cdot  \frac{\cost(C,T)}{|C|^{\alpha/2-1}\costa(C,T)}\ .
    \end{equation*}
    Using Jensen's inequality, we obtain that $|C|^{\alpha/2-1}\costa(C,T) \ge (\cost(C,T))^{\alpha/2}$. Hence we finally get that 

    \begin{equation*}
        \frac{(\alpha+1)^\alpha}{|C|}\sum_{z\in C} \frac{\costa(C,z)}{\costa (C,T)}\cdot \cost (C,T) \le ((\alpha+1)^\alpha g_\alpha) \cdot  \frac{(\cost(C,\mu_C))^{\alpha/2}}{(\cost(C,T))^{\alpha/2-1}}\ .
    \end{equation*}
    From there, if $\cost(C,T)\le (\alpha+1)^2\cdot (g_\alpha)^{2/\alpha}\cost(C,\mu_C)$ then the lemma already holds since adding an additional center can only decrease the cost of $C$. Otherwise, we clearly get that 
    \begin{equation*}
        \frac{(\alpha+1)^\alpha}{|C|}\sum_{z\in C} \frac{\costa(C,z)}{\costa (C,T)}\cdot \cost (C,T) \le ((\alpha+1)^2\cdot (g_\alpha)^{2/\alpha}) \cdot  \cost(C,\mu_C)\ ,
    \end{equation*}
    which finishes the proof.
\end{proof}
\begin{lemma}
\label{lem:cost_alpha_clusters}
    For any cluster $C$, we have that 
    \begin{equation*}
        \costa(C,\mu_C)\le g_\alpha\cdot |C|\cdot (\sigma_C)^\alpha\ . 
    \end{equation*}
\end{lemma}
\begin{proof}
    We note that $\costa(C,\mu_C)\le \frac{1}{|C|}\sum_{z\in C} \costa(C,z)$. Hence, we obtain
    \begin{align*}
        \costa(C,\mu_C) &\le \left(\frac{1}{|C|}\sum_{z\in C} \costa(C,z)\right)\\
        &\le |C|^{1-\alpha/2} \cdot g_\alpha \cdot (\cost(C,\mu_C))^{\alpha/2}= g_\alpha\cdot |C|\cdot (\sigma_C)^\alpha\ ,
    \end{align*}
    where the second inequality uses our assumption.
\end{proof}

We are now ready to analyze the global increase in potential.
\begin{lemma}
\label{lem:potential_increase}
For every $i\ge 0, \alpha>2, t>0$, and any past selection of centers $Z_{t-1}$, we have that 
\begin{equation*}
    \mathbb E\left[\phi_i(t)-\phi_i(t-1)  \mid \tau_i(t)=\tau_i(t-1)+1\right] \le h(\alpha)\cdot  \left(2^i\right)^{1-2/\alpha} \cdot (k_i-\tau_i(t-1))^{2/\alpha} \cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha}\ ,
\end{equation*}
where $h(\alpha)=\frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2}$, and 
\begin{equation*}
    \mathbb E\left[\phi_i(t)-\phi_i(t-1)  \mid \tau_i(t)=\tau_i(t-1)\right] \le 0\ .
\end{equation*}
\end{lemma}
\begin{proof}
    If $\tau_i(t)=\tau_i(t-1)$, then $w_i(t)=w_i(t-1)$ and clearly the potential $\phi_i$ can only decrease. 
    
    If $\tau_i(t)=\tau_i(t-1)+1$ then either $z_t$ belongs to $U_{t-1}^{(i)}$, in which case the potential $\phi_i$ can only decrease in expectation (see Lemma \ref{lem:potential_hit_new}). Therefore there remains only the case that $z_t\in H_{t-1}$. In this case, let us denote by $Z_{t-1}$ the current set of selected centers. Using Lemma \ref{lem:potential_hit_old} we have that

    \begin{align*}
        \mathbb E&\left[\phi_i(t)-\phi_i(t-1) \mid \{\tau_i(t)=\tau_i(t-1)+1,Z_{t-1}\}\right]\\
        &\le (2^i)^{1-2/\alpha} \cdot \frac{\sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}\cdot \frac{\costa(H_{t-1},Z_{t-1})}{\costa(H_{t-1},Z_{t-1})+ \costa(U_{t-1}^{(i)},Z_{t-1})}\\
        &\le (2^i)^{1-2/\alpha} \cdot \frac{\sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}\cdot \frac{\costa(H_{t-1},Z_{t-1})}{\costa(H_{t-1},Z_{t-1})+ |U_{t-1}^{(i)}| \cdot \left(\frac{\sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}\right)^{\alpha/2}}\ ,
    \end{align*}
    where the last inequality uses the concavity of $x\mapsto x^{2/\alpha}$. If we consider the last expression as a function of $X:=\frac{\sum_{C\in U_{t-1}^{(i)}} (\costa (C,Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|}$ (the other quantities being fixed), one can see that this expression attains a maximum value for
    \begin{equation*}
        X=\left(\frac{\costa(H_{t-1},Z_{t-1})}{|U_{t-1}^{(i)}|\cdot (\alpha/2-1)}\right)^{2/\alpha}\ .
    \end{equation*}
    Plugging in this value, we obtain that 
    \begin{align*}
        \mathbb E&\left[\phi_i(t)-\phi_i(t-1)  \mid \{\tau_i(t)=\tau_i(t-1)+1,Z_{t-1}\}\right] \\
        &\le \frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2} \cdot (2^{i})^{1-2/\alpha} \cdot \frac{(\costa(H_{t-1},Z_{t-1}))^{2/\alpha}}{|U_{t-1}^{(i)}|^{2/\alpha}}\\
        &\le  \frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2} \cdot (2^{i})^{1-2/\alpha} \cdot (k_i-\tau_i(t-1))^{-2/\alpha} \cdot \mathbb (\costa(H_t,Z_{t-1}))^{2/\alpha}\ ,
        \end{align*}
    where the second inequality uses the fact that $|U_{t-1}^{(i)}|\ge k_i-\tau_i(t-1)$. By the law of total expectation, we have that
    \begin{align*}
        \mathbb E&\left[\phi_i(t)-\phi_i(t-1)  \mid \tau_i(t)=\tau_i(t-1)+1 \right] = \mathbb E_{Z_{t-1}}\left[\mathbb E\left[\phi_i(t)-\phi_i(t-1)  \mid \{\tau_i(t)=\tau_i(t-1)+1,Z_{t-1}\}\right]\right]\\
        &\le \frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2} \cdot (2^{i})^{1-2/\alpha} \cdot (k_i-\tau_i(t-1))^{-2/\alpha} \cdot \mathbb E_{Z_{t-1}}\left[\left( \costa(H_{t-1},Z_{t-1})\right)^{2/\alpha}\right]\\
        &\le \frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2} \cdot (2^{i})^{1-2/\alpha} \cdot (k_i-\tau_i(t-1))^{-2/\alpha} \cdot  \left( \mathbb E_{Z_{t-1}}\left[\costa(H_{t-1},Z_{t-1})\right]\right)^{2/\alpha}\\
        &\le \frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2} \cdot (2^{i})^{1-2/\alpha} \cdot (k_i-\tau_i(t-1))^{-2/\alpha} \cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha \right)^{2/\alpha}\ ,
    \end{align*}
    where the second inequality uses Jensen's inequality, and the last inequality uses Lemma \ref{lem:cost_alpha_clusters} and Lemma \ref{lem:} (arthur and vassilvitskii).
\end{proof}


\begin{lemma}
\label{lem:potential_global}
For any $\alpha>2$, we have that 
\begin{equation*}
    \frac{\mathbb E\left[\phi(k)\right]}{\OPT} \le f(\alpha) \cdot (g_\alpha)^{2/\alpha} \cdot \left(\frac{\smax}{\smin}\right)^{1-2/\alpha}\cdot  \min \{\ell,\log(k)\}^{2/\alpha}\ ,
\end{equation*}
where $f(\alpha)=\frac{(\alpha/2-1)^{1-2/\alpha}}{\alpha/2-1}$.
\end{lemma}
\begin{proof}
    Using Lemma \ref{lem:potential_increase}, we obtain that 
    \begin{align*}
        \mathbb E\left[ \phi_i(k) \right] &\le h(\alpha)\cdot  \left(2^i\right)^{1-2/\alpha} \cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha} \cdot \sum_{t=0}^{k_i-1} (k_i-t)^{-2/\alpha}  \\
        &\le h(\alpha)\cdot  \left(2^i\right)^{1-2/\alpha} \cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha} \cdot \int_{0}^{k_i} (k_i-u)^{-2/\alpha} du \\
        &\le h(\alpha)\cdot  \left(2^i\right)^{1-2/\alpha} \cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha} \cdot \frac{(k_i)^{1-2/\alpha}}{1-2/\alpha}\ .
    \end{align*}
    Therefore, we obtain  
    \begin{align*}
        \mathbb E[\phi(k)] = \sum_{i\in \mathcal L} \mathbb E[\phi_i(k)] &\le \frac{h(\alpha)}{1-2/\alpha}\cdot \left((2^\alpha g_\alpha) \sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha} \cdot \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &= \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha}\cdot  \left(\sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha} \cdot \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\ .
    \end{align*}
    Comparing this with optimum clustering, we get using basic algebraic manipulations
    \begin{align*}
        \frac{\mathbb E[\phi(k)]}{\OPT} &= \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \frac{\left(\sum_{C}  |C|(\sigma_C)^\alpha\right)^{2/\alpha}}{\sum_{C}  |C|(\sigma_C)^2} \cdot  \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &= \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \frac{\left(\sum_{C}  |C|\left(\frac{\sigma_C}{\smax}\right)^\alpha \smax^\alpha \right)^{2/\alpha}}{\sum_{C}  |C|\left(\frac{\sigma_C}{\smin}\right)^2\cdot \smin^2} \cdot  \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &\le \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \frac{\left(\sum_{C}  |C|\left(\frac{\sigma_C}{\smax}\right)^2 \right)^{2/\alpha}\cdot \smax^2}{\sum_{C}  |C|\left(\frac{\sigma_C}{\smin}\right)^2\cdot \smin^2} \cdot  \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &\le \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \frac{\left(\sum_{C}  |C|\left(\sigma_C\right)^2 \right)^{2/\alpha}\cdot \smax^{2-4/\alpha}}{\sum_{C}  |C|\left(\frac{\sigma_C}{\smin}\right)^2\cdot \smin^2} \cdot  \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &\le \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \frac{\left(\sum_{C}  |C|\left(\frac{\sigma_C}{\smin}\right)^2 \right)^{2/\alpha}\cdot (\smin)^{4/\alpha}\cdot \smax^{2-4/\alpha}}{\sum_{C}  |C|\left(\frac{\sigma_C}{\smin}\right)^2\cdot \smin^2} \cdot  \sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}\\
        &\le \frac{2h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha} \cdot \left(\frac{\smax}{\smin}\right)^{2-4/\alpha}\cdot \frac{\sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}}{\left(\sum_{C}  |C|\right)^{1-2/\alpha}} \\
        &\le \frac{4h(\alpha) (g_\alpha)^{2/\alpha}}{1-2/\alpha}\cdot \left(\frac{\smax}{\smin}\right)^{2-4/\alpha}\cdot \frac{\sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}}{\left(\sum_{i\in \mathcal L}  2^i k_i\right)^{1-2/\alpha}}\ .
    \end{align*}
    To conclude the proof, we need to upper bound the ratio 
    \begin{equation*}
        \frac{\sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}}{\left(\sum_{i\in \mathcal L}  2^i k_i\right)^{1-2/\alpha}}
    \end{equation*}
    for any integer sequence $(k_i)_{i\ge 0}$ satisfying the constraint $\sum_{i\ge 0}k_i=k$. Using Jensen inequality (note that $x\mapsto x^{1-2/\alpha}$ is concave), we immediately obtain 
    \begin{equation*}
        \frac{\sum_{i\in \mathcal L} (2^i k_i)^{1-2/\alpha}}{\left(\sum_{i\in \mathcal L}  2^i k_i\right)^{1-2/\alpha}} \le \ell^{2/\alpha}\ .
    \end{equation*}
    For the second upperbound, note that to have equality in Jensen's inequality, we must have that $2^ik_i=2^jk_j$ for all $i,j\ge 0$ such that $k_i \neq 0, k_j\neq 0$. Intuitively, this can only happen when $\ell =O(\log k)$. TODO formal proof 
\end{proof}

Using Lemma \ref{lem:potential_global} with Lemma \ref{lem:potential_upper_bound} concludes the proof.
